Personalized Parsons Puzzles as Scaffolding Enhance Practice Engagement Over Just Showing LLM-Powered Solutions

As generative AI products could generate code and assist students with programming learning seamlessly, integrating AI into programming education contexts has driven much attention. However, one emerging concern is that students might get answers without learning from the LLM-generated content. In this work, we deployed the LLM-powered personalized Parsons puzzles as scaffolding to write-code practice in a Python learning classroom (PC condition) and conducted an 80-minute randomized between-subjects study. Both conditions received the same practice problems. The only difference was that when requesting help, the control condition showed students a complete solution (CC condition), simulating the most traditional LLM output. Results indicated that students who received personalized Parsons puzzles as scaffolding engaged in practicing significantly longer than those who received complete solutions when struggling.

==> Sections/2_related_work.tex <==
\section{Related work}
\subsection{LLM-based programming assistants in computing classrooms}
After recognizing the ability of LLMs to generate code fixes, natural explanations \cite{kazemitabaar2024codeaid}, and pedagogical conversations \cite{jin2024teach}, significant effort has been invested in creating and evaluating LLM-based programming assistants with diverse content focus and granularity. There are two main types of programming assistants, namely question-answering chat and clicking-for-help. The first type often requires students to ask a meaningful question and then programming assistants will reply with answers and potential next-step action recommendations \cite{lyu2024evaluating, liu2024teaching}. The second type often triggered instructional support to students' existing code with a clickable button, like providing hints \cite{xiao2024exploring}, or direct code fixes \cite{kazemitabaar2024codeaid}. However, most of these approaches are focused on providing text-heavy instructional materials. Such long and plain textual materials could discourage active learning unless students produce active reading and reflection while reading the text \cite{chi2014icap}. Students are also likely to shift to commercialized generative AI tools to get quicker answers \cite{kazemitabaar2024codeaid}. Therefore, \sys{} aims to provide a more active support mechanism that requires students to conduct physical moves to create the final correct solution. This method is expected to increase students' engagement with the practice task.
% \vspace{-3mm}

\subsection{Parsons puzzles as programming support}
In Parsons puzzles, students arrange mixed-up blocks to solve a problem \cite{parsons2006parson}. Typically, the mixed-up blocks are presented separately from the solution area. Students need to drag all the required blocks into the solution area and arrange them there \cite{ericson2022parsons}. There are various Parsons puzzle types. For example, distractors are code blocks that are not part of the correct solution, and can also be added to highlight misconceptions \cite{ericson2022parsons}. \citeauthor{ericson2019investigating} developed two adaptation types in Parsons puzzles: intra-problem and inter-problem adaptation \cite{ericson2019investigating}. Intra-problem adaptation reduces the difficulty of the current Parsons problem, and inter-problem adaptation impacts the next problem's difficulty level based on student’s performance on the current one \cite{ericson2018evaluating}. Learners can initiate the intra-problem adaptation by clicking the "Help Me" button after a certain number of full attempts, and the system will either remove a distractor block or combine two blocks into one. Previous studies investigated the use of a single fully movable Parsons puzzle to support programming \cite{hou2022using}. In fully movable Parsons puzzles, students start with an empty solution area. They must select all the required blocks and arrange them in the correct order to solve the problem. Building on past efforts, \sys{} improved the Parsons puzzles by personalizing the solution based on the student's incorrect code and personalizing the block setups based on students' existing progress. 

% Problems with paired distractors, where learners are instructed to pick the correct block from a visually paired block set with one correct block and one distractor block, are easier to solve than those with unpaired distractors \cite{ericson2022parsons}. 

